Do Deep Neural Networks Suffer from Crowding?

Crowding is a visual effect suffered by humans, in which an object that can be recognized in isolation can no longer be recognized when other objects, called flankers, are placed close to it. In this work, we study the effect of crowding in artificial Deep Neural Networks for object recognition. We analyze both standard deep convolutional neural networks (DCNNs) as well as a new version of DCNNs which is 1) multi-scale and 2) with size of the convolution filters change depending on the eccentricity wrt to the center of fixation. Such networks, that we call eccentricity-dependent, are a computational model of the feedforward path of the primate visual cortex. Our results reveal that the eccentricity-dependent model, trained on target objects in isolation, can recognize such targets in the presence of flankers, if the targets are near the center of the image, whereas DCNNs cannot. Also, for all tested networks, when trained on targets in isolation, we find that recognition accuracy of the networks decreases the closer the flankers are to the target and the more flankers there are. We find that visual similarity between the target and flankers also plays a role and that pooling in early layers of the network leads to more crowding. Additionally, we show that incorporating the flankers into the images of the training set does not improve performance with crowding.

==> conclusions.tex <==
%\section{Conclusion}
%\begin{enumerate}
%\item We analysed the effect of crowding in CNNs and eccentricity dependent networks.
%\item As our models are trained within a supervised learning framework, we also investigate the effects of training with clutter.
%\item We have seen that in standard CNNs, the effect of flankers is uniform across all displacements.
%\item We also see that when flankers are placed closer to the target, they interfere more with recognition.
%\item The statistics of the flanker dataset also affect how much crowding occurs.  Omniglot flankers crowd less than MNIST flankers
%\item In eccentricity-dependent networks, however, we see that the distance from the center of the field of view determines the amount of crowding.
%\item To mitigate this effect, it is necessary to use contrast normalisation.
%\end{enumerate}



==> previous.tex <==
\section{Related Work}
{\bf GR: Maybe we don't need related work if we do a well motivated introduction citing related work there. It's fine to have a related work section as long as (i) we avoid making a list of previous works, (ii) it adds something different from the introduction.}
